Upper Hessenberg and Toeplitz Bohemians

We look at Bohemians, specifically those with population $\{-1, 0, {+1}\}$ and sometimes $\{0,1,i,-1,-i\}$. More, we specialize the matrices to be upper Hessenberg Bohemian. From there, focusing on only those matrices whose characteristic polynomials have maximal height allows us to explicitly identify these polynomials and give useful bounds on their height, and conjecture an accurate asymptotic formula. The lower bound for the maximal characteristic height is exponential in the order of the matrix; in contrast, the height of the matrices remains constant. We give theorems about the numbers of normal matrices and the numbers of stable matrices in these families.

==> ExperimentalResults.tex <==
The methods used for computing the characteristic polynomials and counting the number of eigenvalues presented in Tables~\ref{tab:properties_UHTfulldiagonal}--\ref{tab:nilpotents} will be discussed in detail in a forthcoming paper.  Many of the smaller-dimension computations were done directly in \textsc{Maple} 2017; for instance, computation of the characteristic polynomials of all two million or so matrices in \HH{0}{5}{\{0, {+1}\}} took about six hours on a Surface Pro. The greater number of higher-dimension matrices, or matrices with larger populations, required special techniques and larger \& faster machines.  Eigenvalue computations were also done in \textsc{Matlab} and in Python.  The computed characteristic polynomials are available through the Characteristic Polynomial Database~\cite{CPDB}.

% \#distinct real $\lambda$ &
% 11, 127, 3,229, 180,603


\begin{table}[ht]
    \centering
    \begin{tabular}{ccccc}
        \toprule
        $n$ & \#matrices & \#cpolys &  \#neutral polys & \#neutral matrices \\
        \midrule
         2 & 27 &  16&  2 & 4 \\
         3 & 729  & 166 & 3 & 24 \\
         4 & 59,049 & 3,317 & 7 & 332 \\
         5 & 14,348,907 & 133,255 &  11 & 9,909 \\
         6 & 10,460,353,203 & 10,872,459 & 25 & 696,083 \\
         \bottomrule
    \end{tabular}
    \caption{Some properties of matrices in \HH{0}{n}{\{-1, 0, {+1}\}}. The \#matrices column reports the number of distinct matrices at each dimension.  The \#cpolys column reports the number of distinct characteristic polynomials at each dimension.  The \#neutral polys reports the number of characteristic polynomials where all roots have zero real part.  The \#neutral matrices column reports the number of matrices where all eigenvalues have zero real part.}
    \label{tab:properties_UHTfulldiagonal}
\end{table}
% The following data comes from the
% worksheets tables.mw in the
% Dropbox folder Maple/BohemianExperiments
%
% and cumulativehessenberganalysis.mw
% in the Dropbox folder Maple/BohemianExperiments
%
% \#distinct real $\lambda$ &
%
\begin{table}[ht]
    \centering
    \begin{tabular}{ccccc}
        \toprule
        $n$ & \#matrices & \#cpolys &  \#neutral polys & \#neutral matrices \\
        \midrule
         2 & 3 & 3 & 2 & 2\\
         3 & 27 & 15 & 3 & 6 \\
         4 & 729 & 140 &  7 & 66 \\
         5 & 59,049 & 2,297 & 11 & 1,069 \\
         6 & 14,348,907 & 67,628 & 25 & 45,375 \\
         7 & 10,460,353,203 & 3,606,225 & 45 & 4,105,977\\
         \bottomrule
    \end{tabular}
    \caption{Some properties of matrices in \ZH{0}{n}{\{-1, 0, {+1}\}}. The \#matrices column reports the number of distinct matrices at each dimension.  The \#cpolys column reports the number of distinct characteristic polynomials at each dimension. The \#neutral polys reports the number of characteristic polynomials where all roots have zero real part.  The \#neutral matrices column reports the number of matrices where all eigenvalues have zero real part.}
    \label{tab:properties_UHT(3)}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
         $n$ & multiplicity 1 & ${2}$ & ${3}$ & ${4}$ & ${5}$ & ${6}$\\
         \midrule
         2 & 5 & 1 & & & & \\
         3 & 35 & 0 & 1 & & & \\
         4 & 431 & 5 & 0 & 1 & & \\
         5 & 9,497 & 9 & 3 & 0 & 1 & \\
         6 & 363,143 & 51 & 5 & 1 & 0 & 1 \\
         \bottomrule
    \end{tabular}
    \caption{Number of distinct eigenvalues of various multiplicities of matrices in \ZH{0}{n}{\{-1, 0, {+1}\}}. Most eigenvalues are simple.  It turns out that every multiple eigenvalue also occurs as a simple eigenvalue for some other matrix.  The only $n$-multiple eigenvalue of the class of $n$ by $n$ matrices is, of course, $\lambda = 0$.}
    \label{tab:num_eigs(3)}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{cccccc}
        \toprule
        $n$ & \#matrices & \#cpolys & \#distinct real $\lambda$ & \#neutrals polys & \#neutral matrices \\
        \midrule
         2 & 8 & 6 & 6 & 1 & 1\\
         3 & 64 & 28 & 25 & 1 & 1\\
         4 & 1,024 & 197 & 219 & 1 & 1\\
         5 & 32,768 & 2,235 & 3,264 &  1 & 1\\
         6 & 2,097,152 & 39,768 & 75,045 & 1 & 1\\
         7 & 268,435,456 & 1,140,848 & 2,694,199 & 1 & 1\\
         \bottomrule
    \end{tabular}
    \caption{Some properties of matrices in \HH{0}{n}{\{0, {+1}\}}. The \#matrices column reports the number of distinct matrices at each dimension.  The \#cpolys column reports the number of distinct characteristic polynomials at each dimension.
    The \#distinct real $\lambda$ column reports the number of distinct real eigenvalues in \HH{0}{n}{\{0, {+1}\}}.
    The \#neutral polys reports the number of characteristic polynomials where all roots have zero real part (here only $z^n$). We conjecture that this is always so (and that there is only one matrix for that neutral polynomial).  The \#neutral matrices column reports the number of matrices where all eigenvalues have zero real part.}
    \label{tab:properties_UHT(0-1 poly)}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
         $n$ & multiplicity 1 & ${2}$ & ${3}$ & ${4}$ & ${5}$ & ${6}$ \\
         \midrule
         2 & 6 & 2 & & & & \\
         3 & 43 & 2 & 2 & & & \\
         4 & 413 & 6 & 2 & 2 & & \\
         5 & 6,920 & 6 & 3 & 2 & 2 & \\
         6 & 166,005 & 45 & 6 & 2 & 2 & 2 \\
         \bottomrule
    \end{tabular}
    \caption{Number of distinct eigenvalues of various multiplicities matrices in $\HH{0}{n}{\{0, {+1}\}}$.  Note that in this class of matrices,  diagonal entries of the matrix need not be zero.}
    \label{tab:num_eigs(zero-one)}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
        $n$ & \#matrices & \#cpolys & \#stables & \#neutral polys & \#neutral matrices & \#distinct real $\lambda$ \\
        \midrule
         2 & 8 & 6 & 1 & 1 & 2 & 5\\
         3 & 64 & 32 & 3 & 0 & 0 & 29 \\
         4 & 1,024 & 289 & 14 & 1& 6 & 233 \\
         5 & 32,768 & 4,958 & 93 & 0 & 0 & 	7,363\\
         6 & 2,097,152 & 162,059 & 992 & 2 & 430 & 299,477\\
         7 & 268,435,456 & 10,318,948 & & 0 & 0 &\\
         \bottomrule
    \end{tabular}
    \caption{Some properties of matrices from $\HH{0}{n}{\{-1, {+1}\}}$. The column \#stables reports the number of characteristic polynomials with all roots in the left half plane; the corresponding number of \textsl{matrices} is $1$, $4$, $28$, $424$, and $11,613$. Other columns are as in previous tables. Blank table entries represent unknowns.}
    \label{tab:properties_UHT(Bernoulli)}
\end{table}
\begin{table}[h]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
         $n$ & multiplicity 1 & ${2}$ & ${3}$ & ${4}$ & ${5}$ & ${6}$ \\
         \midrule
         2 & 9 & 1 & & & & \\
         3 & 65 & 0 & 0 & & & \\
         4 & 689 & 5 & 0 & 0 & & \\
         5 & 20,565 & 3 & 0 & 0 & 0 & \\
         6 & 887,539 & 59 & 9 & 1 &  1  & 1 \\
         \bottomrule
    \end{tabular}
    \caption{Number of distinct eigenvalues of various multiplicities of matrices from $\HH{0}{n}{\{-1, {+1}\}}$. The diagonal entries are not zero.}
    \label{tab:num_eigs(Bernoulli)}
\end{table}

Other questions than those answered in these tables can be asked of this data.  For instance, one might be interested in the proportion of singular matrices.  By asking which characteristic polynomials have zero constant coefficient, and counting the number of matrices that have that characteristic polynomial, one can answer such questions. In the case of six by six upper Hessenberg matrices with population $\{-1, {+1}\}$, there are $383,680$ singular matrices, or about $18.3\%$.  Recall that for ``random'' six by six matrices, where the entries are chosen perhaps uniformly over some real interval, the probability of singularity is \textsl{zero} because such matrices come from a set of measure zero.  Yet in applications, the probability of singular matrices is often \textsl{nonzero} because of structure.  By looking at Bohemian matrices, we get some idea of the  influence of structure for finite dimensions~$n$.

